Reparameterization Dependence and Holographic Complexity of Black Holes

We refine the calculation of holographic complexity of black holes in the complexity equals action approach by applying the recently introduced criterion that the action of any causal diamond in static vacuum regions must vanish identically. This criterion fixes empty anti-de Sitter (AdS) spacetime as the reference state with vanishing complexity and renders holographic complexity explicitly finite in all the cases we consider. The cases considered here include the Reissner-Nordstr\"om-AdS black hole, the rotating BTZ black hole, the Kerr-AdS black hole, and AdS-Vaidya spacetime. The criterion is equivalent to imposing that the corner contributions vanish. Contrary to earlier results, we find that the generalized Lloyd bound always holds in the Reissner-Nordstr\"om-AdS and BTZ cases.

==> actionWdW.tex <==
\section{Action on a WdW patch}
\label{actionWdW}

The gravitational action on a WdW patch consists of contributions coming form the bulk of the patch, its boundaries and the joints in which the boundaries meet. Given a bulk action, the variational principle imposes a number of boundary and joint terms. The most familiar case for Einstein gravity is the Gibbons-Hawking-York term \cite{York:1972sj, Gibbons:1976ue}, which applies to space-like or time-like boundaries. When the boundary is not smooth, additional joint terms are necessary \cite{Hartle:1981cf, Hayward:1993my}. In the general case, which includes also null boundaries, the boundary and joint terms have been constructed, \eg in \cite{Parattu:2015gga, Parattu:2016trq, Lehner:2016vdi, Jubb:2016qzt}. We refer to \cite{Jubb:2016qzt} for more references to the original work. We shall now review the contributions one at a time. 

The bulk contribution is given by the Einstein-Hilbert action with a cosmological constant $\Lambda$
%
\begin{equation}
\label{actionWdW:EH}
I_{B} = I_{EH} = \int_{\mathcal{M}}\rmd^D X\sqrt{-g}\,\left(R + \Lambda\right)~.
\end{equation}
%

The boundaries of the patch are hypersurfaces, which one can define in terms of a scalar function $\Phi(X) =0$. In this paper, we use the convention that $\Phi(X)$ is negative inside the patch and positive outside of it. These conventions agree with those in \cite{Jubb:2016qzt, Carmi:2016wjl} and ensure that the one-form $\rmd \Phi$ always points outward.   
If the hypersurface is space-like or time-like, then the unit normal is taken to be  
%
\[ 
   n^\alpha = \frac{\partial^\alpha\Phi}{\sqrt{\left|g_{\alpha\beta}
   \partial^\alpha\Phi\partial^\beta\Phi\right|}}~.
\]
%
In these cases, the boundary contribution to the action is given by the Gibbons-Hawking-York term
%
\begin{equation}
\label{actionWdW:GHY}
I_{S} = I_{GHY} = 2\int_\mathcal{B}\rmd^{D-1} x\sqrt{|h|}\, K~,
\end{equation}
%
where $K = \nabla_\alpha n^\alpha$ is the extrinsic curvature of the boundary, and $h$ is the determinant of the induced metric.

Instead, if the boundary is a null hypersurface, then $\partial^\alpha \Phi$ must be proportional to the null tangent vector,
%
\begin{equation}
\label{actionWdW:vectors}
k^\alpha \equiv \frac{\partial X^\alpha}{\partial\lambda} = e^{\sigma(x)}\partial^\alpha\Phi~.
\end{equation}
%
Here and henceforth, $\lambda$ denotes the hypersurface coordinate that parameterizes the null direction. The function $\sigma(x)$ determines the parameterization of the null direction, \ie the choice of $\lambda$.  
This has been discussed extensively in \cite{Lehner:2016vdi}. 

The analogue of the Gibbons-Hawking-York term is played by\footnote{The different sign with respect to the expression given in \cite{Lehner:2016vdi} derives from different conventions for $k^\alpha$ and $\Phi$.}   
%
\begin{equation}
\label{actionWdW:null}
	I_{N} = 2\int \rmd\lambda\rmd^{D-2} x \sqrt{\gamma}\,\kappa~,
\end{equation}
%
where $\kappa$ is the non-affinity parameter defined by
%
\begin{equation}
\label{actionWdW:kappa}
k^\beta\nabla_\beta k^\alpha = \kappa k^\alpha~.
\end{equation}
%
In \eqref{actionWdW:null}, $\gamma$ is the determinant of the induced metric on the codimension-two space-like part of the boundary that is orthogonal to the null direction.

In addition to the codimension-one boundaries, the WdW patch has also codimension-two joints in which two boundaries intersect. The contribution of a joint depends on the type of the intersecting boundaries. In the case of a joint formed by two null boundaries, it is given by 
%
\begin{equation}
\label{actionWdW:joint}
I_{C} = 2 \epsilon_\mathcal{J} \int_\mathcal{J}\rmd^{D-2} x \sqrt{\gamma}\,\ln\frac{\left|k_1\cdot k_2\right|}{2}~,
\end{equation}
%
where $k_1$ and $k_2$ are the null tangent vectors of the two intersecting boundaries, and the sign $\epsilon_\mathcal{J} = \pm 1$ depends on the relative position of the boundaries and the bulk region. The (convention-dependent) rules can be found in \cite{Lehner:2016vdi, Carmi:2016wjl}. We remark  that there is no real need to memorize these rules, if one does not fix the parameterization functions $\sigma(x)$. As we shall see below, performing an integration by parts in $I_{N}$, one obtains $\sigma$-dependent contributions localized at the joints, which must cancel against the $\sigma$-dependent parts of the joint term $I_{C}$. This determines the signs $\epsilon_\mathcal{J}$.
We refrain from giving the joint terms in the other cases, because we will not need them.

Adding up all these contributions gives an action with a well-defined action principle. Moreover, the full action is additive, \ie one can safely divide a given space-time region into smaller subregions. However, in the presence of null boundaries, it is not invariant under a reparametrization of the null directions, which can be seen from the fact that the arbitrary functions $\sigma(x)$ remain explicit. A remedy is to add a counterterm such that its variation under a reparametrization will cancel the variation of the action. We will use the term suggested in \cite{Lehner:2016vdi}
%
\begin{equation}
\label{actionWdW:ct}
I_{\mathrm{c.t.}} =2\int\rmd\lambda\rmd^{D-2} x\sqrt{\gamma}\, \Theta\ln(\tilde{l}\left|\Theta\right|)~,
\end{equation}
%
where $\Theta$ is the null geodesic expansion. It is defined by $\Theta = \partial_\lambda\ln\sqrt{\gamma}$. The constant $\tilde{l}$ is of dimension length and plays the role of a renormalization scale. 

It has been pointed out in \cite{Jubb:2016qzt} that the choice \eqref{actionWdW:ct} is not unique. There are, in fact, other terms that would serve the same purpose, such as 
%
\begin{equation}
	\label{actionWdW:ct2}
	I'_{\mathrm{c.t.}} =2\int\rmd\lambda\rmd^{D-2} x\sqrt{\gamma}\, \Theta\ln\frac{\rmd\lambda}{\rmd t}~,
\end{equation}
%
where $t$ is an arbitrary affine parametrization, or
%
\begin{equation}
	\label{actionWdW:ct3}
	I''_{\mathrm{c.t.}} =2\int\rmd\lambda\rmd^{D-2} x\sqrt{\gamma}\, \Theta\ln s_{ab}s^{ab}~,
\end{equation}
%
where $s_{ab}$ is the shear tensor of the null geodesic congruence.
We will use the term \eqref{actionWdW:ct} because, as it turns out, \eqref{actionWdW:ct2} is not compatible with the additive properties of the action, while \eqref{actionWdW:ct3} is not regular on the surfaces we need to study.


==> unused.tex <==

Unfortunately, the 
It is difficult to discuss the sign of the integrand in \eqref{kads:Cddot} from the expression \eqref{kads:Gdef}. We can however identify a region of the domain of the function $G(r,\theta)$ in which it may be negative. If we restrict ourselves to $\theta = \frac{\pi}{2}$, \eqref{kads:Gdef} gives
%
\begin{align}
	\label{kads:Gpi/2}
	G\left(r,\frac{\pi}{2}\right) = -\frac{\Delta_r}{2Q}\left(2+\frac{6r^2}{L^2}-(\partial_r \Delta_r) \partial_r \ln \frac{\Pi(\frac{\pi}{2})}{r^2} 
	- \Delta_r \partial_r^2 \ln \frac{\Pi(\frac{\pi}{2})}{r^2}+2a^2\frac{\Pi(\frac{\pi}{2})-\Delta_r r^2}{r^2\Pi(\frac{\pi}{2})}\right)~,
\end{align}
%
where
%
\begin{equation}
	\Pi\left(\frac{\pi}{2}\right) = (r^2+a^2)^2-a^2\Delta_r~.
\end{equation}
%
Remembering that $r_-<r_m(\theta)<r_+$, every factor of the form $-\Delta_r$ that appears in \eqref{kads:Gpi/2}, is positive. This also implies that $\Pi(\frac{\pi}{2})$ is positive too. Then, out of the five terms in the brackets, three are positive. The sign of the other two terms depends on the sings of the functions $\partial_r\ln\frac{\Pi}{r^2}$ and its derivative. Graphical methods can now become useful. Plotting the function $\partial_r\ln\frac{\Pi}{r^2}$ in the interval $r_-<r<r_+$ (Fig.\ref{fig:log_plot}), we can see that the function is positive near $r_-$, while it can be either positive or negative near $r_+$, depending on the parameters values. We also note that the function is always decreasing, making the $\partial_r^2\ln\frac{\Pi}{r^2}$ term in \eqref{kads:Gpi/2}, always negative. Focusing our discussion near $r_+$ for example, where $\partial_r\Delta_r>0$, we can say that the third term of \eqref{kads:Gpi/2} can be either positive or negative, while the forth term is assured to be negative, and these are the contributions that could result in a negative integrand for \eqref{kads:Cddot}. 
%
\begin{figure}
	\centering
	\begin{subfigure}{0.70\textwidth}
		\includegraphics[width = 1\linewidth]{figures/log_plot}
		\caption{$\frac{a}{L} = 0.1$}
	\end{subfigure}
	\begin{subfigure}{0.70\textwidth}
		\includegraphics[width = 1\linewidth]{figures/log_plot2}
		\caption{$\frac{a}{L} = 0.25$}
	\end{subfigure}
	\caption{Plot of the function $\partial_r\ln\frac{\Pi(\frac{\pi}{2})}{r^2}$ for different values of the angular momentum parameter. $m = L$ for all plots.\label{fig:log_plot}}
\end{figure}
%
To find a definitive answer for the sign of the second derivative of the complexity, one should perform the integral in \eqref{kads:Cddot}, however, lacking an explicit expression for the functions $r_m^\pm(\theta)$, this is impossible. What is possible, is to compute the integral in the late time limit $\tau\rightarrow\infty$.

